SelfMix: Robust Learning Against Textual Label Noise with Self-Mixup Training

The conventional success of textual classification relies on annotated data, and the new paradigm of pre-trained language models (PLMs) still requires a few labeled data for downstream tasks. However, in real-world applications, label noise inevitably exists in training data, damaging the effectiveness, robustness, and generalization of the models constructed on such data. Recently, remarkable achievements have been made to mitigate this dilemma in visual data, while only a few explore textual data. To fill this gap, we present SelfMix, a simple yet effective method, to handle label noise in text classification tasks. SelfMix uses the Gaussian Mixture Model to separate samples and leverages semi-supervised learning. Unlike previous works requiring multiple models, our method utilizes the dropout mechanism on a single model to reduce the confirmation bias in self-training and introduces a textual-level mixup training strategy. Experimental results on three text classification benchmarks with different types of text show that the performance of our proposed method outperforms these strong baselines designed for both textual and visual data under different noise ratios and noise types. Our code is available at https://github.com/noise-learning/SelfMix.

==> content/evaluation.tex <==
\section{Analysis and Discussion}
\textcolor{blue}{Add a few sentences to introduce the main content of this section.}

In this section, we
\subsection{Ablation Study}
We remove each sub-method used in SelfMix respectively and check the test accuracy to see whether each component of our proposed method contributes to the task. 
The result is shown in Table ~\ref{table:ablation}.
Since the performance under high noise ratio and insufficient data is worse according to Table ~\ref{table:asym}, we do experiments on small datasets with 5000 samples (Trec has 5452 samples) under 40\% noise ratio of asymmetric noise. 
We observe that each sub-method can make significant contribution to the model's performance.

\subsection{Extensive Application}
To verify the effectiveness of our proposed SelfMix on other pre-trained language models, we also do experiments based on RoBERTa (Table ~\ref{table:roberta}).

\begin{table}\small
  \centering
\renewcommand{\arraystretch}{1.2}
  \renewcommand\tabcolsep{2.5pt}
  \label{tab:freq}
  \begin{tabular}{lc|c|cc|cc}
    \toprule
    Dataset&& Trec &\multicolumn{2}{c|}{AG-News}&\multicolumn{2}{c}{IMDB}\\
    \midrule
    Noise type & & asym & asym & idn & asym & idn \\
    \bottomrule
    \hline
    \multirow{2}*{RoBERTa} & best & 92.12 & 90.54&74.09  & 92.74& 72.49\\
                        & last & 86.56 & 80.60&60.50  & 89.43& 69.94\\
    \hline
    \multirow{2}*{RoBERTa+Ours}  & best & &92.10 & 92.19 & & 84.44\\
                            & last & &73.50 & 92.10 & & 82.87\\               
  \bottomrule
\end{tabular}
  \caption{Test performances with RoBERTa as the base model under 40\% asymmetric/instance-dependent noise.}
\label{table:roberta}
\end{table}

\subsection{The Influence to Model Training}
We record the test accuracy for every few mini-batches and show the learning process on AG-News (120k samples) and IMDB (45k samples) in Figure \ref{fig:process}. 
The left side of the green vertical dotted line is the warm-up stage of SelfMix, which is exactly the same as the base model. 
From the right side of the curve, we can see that the base model reaches peak performance quickly, followed by heavily overfitting the noise data, while SelfMix learns continuously and performs consistently well.
In addition, due to the sample selection at the beginning of each epoch and the label guessing strategy in self-training, the noise ratio in the semi-supervised stage is low, thus SelfMix also stabilizes the training process.

\begin{figure}
	\centering
	\subfigure[40\% asym]{
		\begin{minipage}[t]{0.5\linewidth}
			\centering
			\includegraphics[width=1.5in]{image/train_process.pdf}
		\end{minipage}
	}%
	\subfigure[40\% idm]{
		\begin{minipage}[t]{0.5\linewidth}
			\centering
			\includegraphics[width=1.5in]{image/train_process.pdf}
		\end{minipage}
	}
	\centering
	\caption{The training process on AG-News and IMDB under 40\% asymmetric/instance-dependent noise.}
	\label{fig:process}
\end{figure}

